Tackling Interpretability in Audio Classification Networks with Non-negative Matrix Factorization

This paper tackles two major problem settings for interpretability of audio processing networks, post-hoc and by-design interpretation. For post-hoc interpretation, we aim to interpret decisions of a network in terms of high-level audio objects that are also listenable for the end-user. This is extended to present an inherently interpretable model with high performance. To this end, we propose a novel interpreter design that incorporates non-negative matrix factorization (NMF). In particular, an interpreter is trained to generate a regularized intermediate embedding from hidden layers of a target network, learnt as time-activations of a pre-learnt NMF dictionary. Our methodology allows us to generate intuitive audio-based interpretations that explicitly enhance parts of the input signal most relevant for a network's decision. We demonstrate our method's applicability on a variety of classification tasks, including multi-label data for real-world audio and music.

==> by-design.tex <==
\label{experiments:by-design}



\subsection{Experimental settings}

Most of the settings remain the same for by-design experiments as previously for post-hoc interpretations. We experiment on the same datasets as before. The audio representation and the learnt dictionaries also remain unchanged. Our network architectures too, remain intact, including the selected hidden layers. However, there are couple of modifications. Unlike previously, the classifier is not trained on the datasets and our hyperparameters are slightly different, which are summarized in table \ref{hyperparams:bd}.  

In terms of evaluation there are significant changes. The faithfulness metric is much less significant here. This is because the final classification output is generated by the interpreter itself and thus faithfulness is ensured by-design. The classification performance of our interpreter is now the primary metric. We compare this with several baselines to (i) benchmark performance of our by-design interpretable network, and (ii) to evaluate the modifications introduced in the learning problem while transitioning from post-hoc interpretation to by-design interpretation (section \ref{approach:by-design}).

We now list the baselines used for benchmarking and the goal behind including them:
\begin{itemize}
    \item Audio prototypical networks (APNet) \cite{apnet} act as a primary baseline from literature. It is an audio processing by-design interpretable network. While it generates interpretation differently from us, it is the only system in the literature addressing by-design interpretation for audio modality. Note that the dedicated post-hoc interpretation systems VIBI and SLIME are not relevant for this problem. We utilize their source code for implementation. For fair comparison, we use the same number of prototypes in their network as our number of components.  

    \item In order to ascertain that using a CNN based representation for NMF offer advantage over typical NMF based representations in terms of prediction performance, we also evaluate performance of two NMF variants: Unsupervised NMF based classification and the Task-driven Dictionary Learning (TDL)-NMF model \cite{bisot2017feature}. The unsupervised NMF model simply learns a dictionary on training data, computes average time activations on test samples and makes predictions using a linear model. The TD-NMF model instead updates the initial learnt dictionary with classification loss from the linear model and thus learns them jointly. To implement them, we rely on their source code \ref{}. For both the systems, we experiment with use of two data types to learn NMF-dictionaries. The first is log-magnitude spectrograms and second is power mel-spectrogram (with a square root transformation). We vary dictionary sizes from 64 to 512 components.  

    \item Given the framework level similarities between FLINT and L2I, we also evaluate the performance of the FLINT interpreter when trained for by-design interpretation. As before, we again emphasize that FLINT is not suitable for audio interpretations, but provides a interpretable network design for comparison of performance.  

    \item Variants of L2I: We denote our proposed version of L2I for by-design interpretation as $\textrm{L2I}_{\textrm{BD}}$ w/ $\Theta_{\textsc{att}}$. We further evaluate two variants of our proposed classification network $g(x)$. The first variant ``$\textrm{L2I}_{\textrm{BD}}$-NoPred" does not include a classification loss applied to $f(x)$ and instead applies it directly to $g(x)$. The second variant ``L2I-PostHoc" is simply the interpreter trained for post-hoc interpretation. We compare with these variants to gain perspective on effect of differences between our formulations of post-hoc and by-design problems.  
\end{itemize}

\begin{table}
    \setlength{\tabcolsep}{6pt}
	\centering
	%\small
    \resizebox{0.4\textwidth}{!}{%	
	\begin{tabular}{l c c c c c} 
		\toprule
		  Dataset & $\gamma$ & $\alpha$ & $\beta$ & $K$ & \# of epochs \\ [0.5ex] 
		\midrule 
            ESC-50 & 1.0 & 3.0 & 0.2 & 100 & 51 \\
            %L3 \cite{lll} & 79.8 & $\times$ & $\times$ \\
            SONYC-UST & 1.0 & 4.0 & 0.2 & 80 & 21 \\
            OpenMIC-2018 & 1.0 & 3.0 & 0.2 & 300 & 21 \\
            \bottomrule
	\end{tabular}
     }
	\caption{Hyperparameters for all datasets for by-design interpretation}
    \label{hyperparams:bd}
\end{table}

\subsection{Results}

The performance of all systems is given in Tab. \ref{performance_all}. We compute the same metrics as used to evaluate the classifiers for each dataset. Mean performance along with variance across 3 runs is reported. We make the following key observations:
\begin{itemize}
    \item Among the interpretable neural networks for audio, L2I w/ $\Theta_{\textsc{ATT}}$ clearly outperforms APNet. The size of the models plays an important role in this. L2I learns with the help of a network architecture that feeds it with higher quality representations for prediction compared to architecture in APNet. It is able to sustain a comparable performance w.r.t the base network while imposing an interpretable structure for final prediction model.

    \item L2I comparison with NMF baselines. TD-NMF performs better than unsupervised NMF. This also highlights a unique advantage of combining NMF representations with deep network representations, wherein, the NMF structure leads to interpretability and using deep networks as source provides higher performance compared to directly using NMF activations generated from input for prediction.   

    \item We also validate our design of loss function to train the by-design interpretable network $g(x)$, by comparing it with the two variants of proposed system, L2I-PostHoc and L2I-NoPred. L2I-NoPred performs the worst among the three, highlighting the benefits of updating the hidden layers of $f$ with classification loss imposed on $f(x)$ rather than on $g(x)$. While L2I-PostHoc and $g(x)$ are not directly comparable as hidden layers of $f$ are already trained on classification loss and fixed in the former, this potentially why $g(x)$ tends to perform better as the hidden layers are also updated with joint optimization of all the losses.  
\end{itemize}

\begin{table*}
    \setlength{\tabcolsep}{7pt}
	\centering
	%\small
    \resizebox{0.71\textwidth}{!}{%	
	\begin{tabular}{l c c c} 
		\toprule
		& \multicolumn{1}{c}{ESC-50 (in \%)} & \multicolumn{1}{c}{SONYC-UST} & \multicolumn{1}{c}{OpenMIC-2018}\\
		\cmidrule[1pt](lr){2-2}
            \cmidrule[1pt](lr){3-3}
            \cmidrule[1pt](lr){4-4}
		System & accuracy & macro-AUPRC & avg-weighted-F1 \\ [0.5ex] 
		\midrule
		$\textrm{L2I}_{\textrm{BD}}$ w/ $\Theta_{\textsc{att}}$ & \textbf{70.1 $\pm$ 1.5} & \textbf{0.581 + 0.008} & \bf{0.825 $\pm$ 0.005}\\ 
            APNet \cite{apnet} & 63.6 $\pm$ 1.7  & 0.422 $\pm$ 0.012 & 0.563 $\pm$ 0.025 \\
            %\midrule
            Unsupervised-NMF & 39.4 $\pm$ 2.3 & 0.373 $\pm$ 0.006 & 0.659 $\pm$ 0.018\\
            TD-NMF \cite{bisot2017feature} & 46.7 $\pm$ 2.7 & 0.431 $\pm$ 0.018 & 0.699 $\pm$ 0.012\\
            L2I--Posthoc & 65.4 $\pm$ 3.4 & 0.567 $\pm$ 0.007 & \textbf{0.825 $\pm$ 0.003}\\
            $\textrm{L2I}_{\textrm{BD}}$--NoPred & 64.4 $\pm$ 1.1 & 0.563 $\pm$ 0.004 & 0.746 $\pm$ 0.006\\
            \midrule
            FLINT \cite{flint} & 75.3 $\pm$ 3.6 & 0.556 $\pm$ 0.008 & 0.827 $\pm$ 0.002 \\
            BASE-$f$ & 82.5 & 0.601 & 0.831\\
            %\midrule
 		\bottomrule
	\end{tabular}
     }
	%\vspace{-3pt}
	\caption{Classification performance for by-design interpretation on all three datasets. The evaluated systems include our proposed by-design interpretable network, denoted as $\textrm{L2I}_{\textrm{BD}}$ w/ $\Theta_{\textsc{att}}$, its variant with modified loss function ($\textrm{L2I}_{\textrm{BD}}$--NoPred), interpreter trained for post-hoc interpretation (L2I--Posthoc), classification models based on traditional NMF (unsupervised NMF and TD-NMF) and audio prototypical network APNet. The classification network pre-trained for performance for post-hoc interpretation (BASE-$f$) and FLINT are used as references for high performance networks not suitable for audio interpretation.}
    \label{performance_all}
\end{table*}


==> ideas_notes.tex <==
\begin{itemize}
    \item Can add algorithm for explanation generation, component selection
\end{itemize}



% Ideas for modifying the for journal

Modify introduction by directly motivating the example, interpretation approaches could be discussed in related works.

Add by-design papers to references. Expand with more references.

Modifying system description: (1) Combine by-design and post-hoc single figure for that, (2) Present as done in presentation and poster by getting rid of discussing NMF at the start (3) Also refer to FLINT






% Idea for abstract

Write about the broad idea + losses

Connecting hidden layer representations to component activations. 


% Ideas for introduction
Use of neural networks in decision-critical domains has necessitated interpreting their decisions in terms of high-level concepts. In this work we concern ourselves with post-hoc interpretation of deep neural networks for audio. While several works have tackled visual and text modality, work on audio has been relatively limited. Although explanations in terms of high level concepts is desired, a key missing ingredient from existing audio interpretability literature is the ability to provide audio-based interpretations. Let us consider an example to understand this better. Suppose an audio classification network that is performing event detection on a street sound file recognizes a dog bark event. An ideal interpreter for this classification decision would have the ability to not only localize the dog bark but also be able to present this as an audio signal with most relevant parts emphasized. 

Humans parsing an audio scene, typically



%NMF intro
Given a magnitude or power spectrogram $\Va$ containing $F$ frequency bins and $N$ time frames, we use NMF to decompose it into a product of two non-negative matrices, such that,
\[\Va \approx \Wa\Ha\]

Here, $\Wa = [\Wak{1}, \Wak{2}, \ldots, \Wak{K}]$ is interpreted as the dictionary matrix containing $K$ components and $\Ha = []$ a matrix containing the corresponding time activations.

Conciseness, class-components analysis map, ...

One can listen to individual components, but also to their sum. Thus, number of single components can be more than 2-3...

Pay attention to the non-explained example, comment on them, listen them.



%Outline

Introduction
 - Motivation
 
 (1) Crucial aspect of interpretability is understandability for user -> 
 (2) Traditional approaches mostly attribution techniques -> 
 (3) Requirement of understandability pushed more methods for different units of interpretation (logical rules, prototypes, concepts) -> 
 (4)(a) However most of these methods suitable for tabular and image modalities. Not suitable for audio processing networks as image-based explanations are not understandable even for experts?
 (4)(b) Similar type of push for explaining graph neural networks ->
 (5) Main motivation of listenable explanations for audio networks. We tackle the post-hoc explainability 
 (6) Intro about our system -- include that we opt for setting of FLINT?
 
 
 - Contributions
 
 
Related works
 - Interpretabiity for audio
 
 - Concept based interpretability
 
 - Link with NMF
 
 
 
System Design

 - ADD "interpreter module $\bmI$" in figure

 - Problem formulation

   + Design of psi
 - Now discuss interpreter design
   + Design of theta
   + NMF usage within our system + dictionary learning (fix W)
   + Loss function
 
 - Learning algorithm
   + Steps of learning (algo)

 - Interpretation generation
   + Algorithm to generate


Experiments
 - Baselines
 
 - Classification network description
 
 - Audio pre-processing/params + Hyperparameters
 
 - Quantitative metrics
   + Fidelity
   + Faithfulness?
   
 - Experiment on ESC-50
   + Dataset description
   + Quantitative results (classification accuracy)
   + Interpretability evaluation (Noise experiments)
   + Faithfulness eval
   
 - Experiment on SONYC-UST
   + Dataset description
   + Quantitative results (AUPRC metrics, DCASE)
   + Qualitative results
   + Faithfulness eval

 
 


% Tables

 2 tables, 1 in ESC-50, 1 in SONYC-UST
 
 ESC-50 table
 
 Columns contain metrics top-1, top-3, top-5
 
 Rows contain names for systems implemented 
 
 
 Same pattern for SONYC-UST but replace column names my macro-AUPRC, micro-AUPRC, max-F1
 
 The column names for both tables can be under a header of fidelity






















% Points for rebuttal
(1) Generating audio explanations from inverting AM+PI maps of FLINT

(2) log-mag spectrogram usage over mag spectrogram 

(3) Faithfulness results on other folds of ESC-50

(4) SLIME baseline

Our method L2I and SLIME are similar in two aspects: (1) In motivation to address interpretability beyond common image interpretability based methods, (2) Generation of listenable interpretations. The two methods fundamentally differ from each other in almost every technical aspect. SLIME uses LIME as the base method to generate interpretations with a novel simplified representation of explicitly dividing the input into time/frequency/time-frequency blocks. The hyperparameters of SLIME (number of divisions, number of selected blocks in the interpretations) are thus to an extent target class and sample dependent. In contrast the hyperparameters for L2I are global and not sample dependent. L2I requires training time to train an interpreter that approximates the network globally. SLIME on the other hand builds an interpreter for each sample separately in its neighborhood. Thus, L2I requires training time which SLIME does not. However, once trained, for an individual sample L2I generates interpretations significantly faster than SLIME.    

(5) Subjective evaluation

(6) Improve system?

(7) Pooling of theta why wasn't max your preferred system over attention

(8) Your system is too similar to FLINT


(9) Code not shared
We plan to make our code public on github upon publication.

(10) Hyperparameter tuning of $\alpha, \beta$ not shared
Experiment on SONYC-UST
(reconstruction loss, output fidelity loss, macro-AUPRC, micro-AUPRC)
$\alpha=10.0, \beta=0.8, 0.028, 0.386, 0.900, 0.914$
$\alpha=1.0, \beta=0.8, 0.045, 0.375, 0.921, 0.938$
$\alpha=100.0, \beta=0.8, 0.027, 0.445, 0.612, 0.756$
$\alpha=10.0, \beta=8.0, 0.048, 0.386, 0.879,  0.922$
$\alpha=10.0, \beta=0.08, 0.028, 0.388, 0.876, 0.921$

High $\alpha$ results in poor fidelity performance and only slightly better reconstruction performance. Small $\alpha$ results in poorer reconstruction performance and only slightly better fidelity performance. $\alpha$ was chosen to bring the two losses on a similar scale. High $\beta$ negatively affects reconstruction error. Didn't vary $\beta$ much from 1.   

(11) K time and memory problem

(12) Hidden layer ablation
Experiment on ESC-50 fold 1
$3 blocks, 0.079, 1.546, 65.5$
$2 blocks, 0.103, 1.572, 61.5$
$1 block, 0.118, 1.698, 57.8$

(13) K experiment
$K=10, 0.136, 2.416, 39.3, 199s, 894s$
$K=40, 0.104, 1.647, 62.5, 421s, 888s$
$K=70, 0.093, 1.605, 62.0, 601s, 893s$
$K=100, 0.079, 1.546, 65.5, 700s, 905$
$K=128, 0.083, 1.544, 64.5, 789s, 960$





% Backup of old pointers written in paper

Need for audio-based interpretations -- Lack of such capability in existing methods -- position with respect to interpretability literature -- use of NMF-based dictionary learning in audio and its advantages as an interpretable system %-- Our framework and its contributions

{\bf Contributions (Minor \& Major)}

\begin{itemize}
    \item \hl{Linking NMF and deep network representations} (contribution for ML community in general)
    
    \item Considerably more meaningful \& novel interpretability for audio  -- In terms of \hl{high-level audio objects, listenable for end-user} (contribution for interpretability and audio community)
    
    \item \hl{Multi-label classification task + Real-world difficult dataset} for application (multi-labelled tasks are rare for interpretability, application to real world data attractive for interpretability and audio community)
    
    \item Potentially widely \hl{applicable for different types of audio inputs such as generic sound events, music, speech}
    
    \item Potential \hl{faithufulness evaluation + interesting subjective evaluation designs} (small contribution for interpretability)
    
    \item Popular networks being interpreted (interesting for audio community)
\end{itemize}

%



We present the faithfulness results in Table \ref{faithfulness_esc50}. We report the median faithfulness over the test set $\textrm{FF}_{\textrm{median}}$ for our primary system L2I + $\Theta_{\textsc{ATT}}$ at different levels of threshold $\tau$. Smaller $\tau$ corresponds to more number of components being considered relevant. We also report $\textrm{FF}_{\textrm{median}}$ for baseline with random selection of components being removed not considered relevant. However, we report its results with the lowest threshold,



%Things to do:
- two equation/notation errors h_k transpose and L c, x expression (done)
- Discussion regarding FLINT. (done)
- INVASE, time-series methods references (done)
- Incorporate R1 references regarding NMF (done)
- Table 1: Neither FLINT and VIBI give audio-based interpretations. (done)

- Add subjective evaluation (ongoing)

- Ask about keywords: audio interpretability, post-hoc explainability, non-negative matrix factorization.

- Key main para to justify our evaluation strategy. (a) Clearly point out the relevance of question posed to the user in subjective evaluation and usage of a baseline, (b) Faithfulness evaluation compared to random baseline useful, (c) descriptions on website

- We use source separation/enhancement in the motivation. The ESC-50 qualitative experiment can be confused with denoising task. Denoising and enhancement are related \textbf{BUT NOT} the main tasks. Neither the expected output is supposed to correspond to these tasks nor is the input suitable for them. Likely possibility that network does not highly activate everywhere object of interest is present, so only hearing part of object strongly is possible. The network could also be detecting noise in some cases (in most we can't confirm this). This significantly makes interpretation task different from denoising or enhancement. However these goals aid understandability while listening. Also note that the input to the interpreter is hidden layers of network trained for classification performance, not the spectrogram itself, so it is unreasonable to expect interpreter to operate as a high-performance denoising or source separation/enhancement system. (b) Reduction in level of noise in the input

- In case of ESC-50 exp, specify network never trained with noisy samples

- network is pre-trained specify in multiple places

- Create space in main paper by moving details to supplementary (ongoing)

- Better examples on website
- More qualitative description on the website, maybe also highlight differences between interpretation and denoising and enhancement.
- Clustering (done, for supp?) -- SONYC-UST
- Add hyperparams exps in appendix
- Misclassification samples (for supp, to be added)
- Overlapping sounds samples in ESC-50? 
- Metric to measure noise?


%sec 3
---------------------------
- code


==> results.tex <==
% Intended organization


\subsection{Datasets}
We experiment with three datasets covering different types of learning tasks, source data etc. We discuss each of them in greater detail below. 
\subsubsection{ESC50}: ESC-50 \cite{esc50} is a popular benchmark for environmental sound classification task. It is a multi-class dataset that contains 2000 audio recordings of 50 different environmental sounds. The classes are broadly arranged in five categories namely, animals, natural soundscapes/water sounds, human/non-speech sounds, interior/domestic sounds, exterior/urban noises. Each clip is five-seconds long and has been extracted from publicly available recordings on the \texttt{freesound.org} project. The dataset is prearranged into 5 folds.

\subsubsection{SONYC-UST}: The DCASE task used a very challenging real-world dataset called Sounds of New York City-Urban Sound Tagging (SONYC-UST) \cite{cartwright2019sonyc}. It contains audio collected from multiple sensors placed in the New York City to monitor noise pollution. It consists of eight coarse-level and 20 fine-level labels. We opt for the coarse-level labeling task that involves multi-label classification into: `engine', `machinery-impact', `non-machinery-impact', `powered-saw', `alert-signals', `music', `human-voice', `dog'. 
%The dataset consists of 13500 training samples and 664 test samples. It suffers from class imbalance, which we mitigate through class-wise weighting of the loss function. Furthermore, while the testing data has been annotated by experts, each training data point has been labeled by three volunteers. We use minority voting to obtain the final ground-truth labels for training \cite{cartwright2019sonyc}. 
This task is highly challenging for several reasons: (i) since it is real-world audio, the samples contain a very high level of background noise, (ii) the audio sources corresponding to the classes are often weak in intensity, as they are not necessarily close to the sensors, (iii) some classes may also be highly localized in time and more challenging to detect, (iv) lastly, noisy audio also makes it difficult to annotate, leading to labeling noise. This is especially true for training data that was labeled by volunteers.

\subsubsection{OpenMIC-2018}: The OpenMIC-2018 dataset \cite{openmic} is composed of 20000 polyphonic audio recordings annotated with weak labels from among 20 instrument classes. The dataset was created by querying the content available on Free Music Archive under the Creatives Commons license with AudioSet concept ontology and using a multi-instrument estimator model trained on AudioSet data to suggest candidates for annotation. Each recording/clip is 10 seconds long. A single sample generally consists of weak labels of only a small subset of classes. Each instrument class has at least 500 positive and 1500 total annotated samples. Compared to SONYC-UST, the number of positive samples intra class and inter class are considerably more balanced. It is currently the only large publicly available dataset with multi-label annotation for polyphonic audio. 



\subsection{Implementation details}
\subsubsection{Classification network} We interpret a VGG-style convolutional neural network proposed by Kumar et al. \cite{kumar_wft}. This network was chosen due to its popularity and applicability for various audio scene and event classification tasks. It can process variable length audio and has been pretrained on AudioSet \cite{audioset}, a large-scale weakly labeled dataset for sound events. It takes as input a log-mel spectrogram. The architecture broadly consists of six convolutional blocks (B1--B6) followed by a convolutional layer with pooling for final prediction. Most convolutional blocks consist of two sets of conv2D + batch norm + ReLU layers followed by a max pooling layer. We fine-tune this network on each dataset separately before training our system for any post-hoc interpretations. For ESC-50, we modify only fully-connected layers after the convolutional blocks while for SONYC-UST and OpenMIC-2018, we modify all the layers during fine-tuning. 

\noindent \textbf{Classifier performance}.~ On ESC-50, the classifier is evaluated using 5-fold cross-validation. It achieves an accuracy of $82.5 \pm 1.9$\% over the 5 folds, higher than the average human accuracy of 81.3\%. SONYC-UST is an unbalanced multi-label dataset. The evaluation is done using AUPRC based metrics. Our fine-tuned classifier achieves a macro-AUPRC (official metric for DCASE 2020 challenge) of $0.601$. This is higher than the DCASE baseline performance of 0.510 and comparable to the best performing system macro-AUPRC of 0.649 \cite{Arnault2020}. Note that it is obtained without use of data augmentation or additional strategies to improve performance. OpenMIC-2018 is a relatively balanced multi-label dataset. To evaluate our trained classifier, we use the weighted average F1-score metric, proposed in the original paper. The metric computes for each class a weighted average of F1-scores over the positive and negative samples. The final score is the average over 20 classes. Our classifier achieves final score of 0.83, better than the VGGish based baseline score of 0.78 and competitive with other recent models. These details are tabulated in Tab. \ref{benchmark_f}. As noted earlier, the pre-training is only executed for post-hoc interpretations.

\begin{table}
    \setlength{\tabcolsep}{3pt}
	\centering
	%\small
    \resizebox{0.49\textwidth}{!}{%	
	\begin{tabular}{l c c c} 
		\toprule
		& \multicolumn{1}{c}{ESC-50 (in \%)} & \multicolumn{1}{c}{SONYC-UST} & \multicolumn{1}{c}{OpenMIC-2018}\\
		\cmidrule[1pt](lr){2-2}
            \cmidrule[1pt](lr){3-3}
            \cmidrule[1pt](lr){4-4}
		System & top-1 & macro-AUPRC & avg-weighted-F1 \\ [0.5ex] 
		\midrule 
            Human accuracy \cite{esc50} & 81.3 & $\times$ & $\times$ \\
            ESC50-CNN baseline \cite{esc50} & 64.5 & $\times$ & $\times$ \\
            %L3 \cite{lll} & 79.8 & $\times$ & $\times$ \\
            Arnault et al. \cite{Arnault2020} & $\times$ & 0.649 & $\times$ \\
            Koutini et al. \cite{bl2_omic} & $\times$ & $\times$ & 0.822 \\
            VGGish \cite{sonyc_ust, openmic} & $\times$ & 0.510 & 0.785 \\
            \midrule
            Current-$f$ & 82.5 & 0.601 & 0.831 \\
 		\bottomrule
	\end{tabular}
     }
	\caption{Benchmarking performance of pre-trained classifier $f$ for post-hoc interpretation.}
    \label{benchmark_f}
\end{table}

\subsubsection{Audio time-frequency representation} For both the tasks, we perform the same audio pre-processing steps. All audio files are sampled at 44.1kHz. STFT is computed with a 1024-pt FFT and 512 sample hop size, which corresponds to about 23ms window size and 11.5ms hopsize. The log-mel spectrogram is extracted using 128 mel-bands.

\subsubsection{Dictionary learning} The matrix on which we apply sparse-NMF to learn $\Wa$, $\Va_{\text{train}}$, is constructed differently for each dataset due to their specific properties. For ESC-50,  $\Va_{\text{train}}$ is constructed by concatenating the log--magnitude spectrograms corresponding to each sample in the training data of the cross-validation fold (1600 samples for each fold). SONYC-UST however, is an imbalanced multilabel dataset with very strong presence of background noise. A procedure to learn components, as for ESC-50, yields many components capturing significant background noise, affecting understandability of interpretations. Hence, we process this dataset differently. We first learn $\Wa_{\text{noise}}$, that is, a set of 10 components to model noise using training samples with no positive label. Then, for each class, we randomly select 700 positively-labeled samples from all training data and learn 10 new components (per class) with $\Wa_{\text{noise}}$ held fixed for noise modeling. All $10 \times 8=80$ components are stacked column-wise to build our dictionary $\mathbf{W}$. While this strategy helps us reduce the number of noise-like components in the final dictionary, it does not completely avoid it. OpenMIC is instead a balanced multilabel dataset for rare noise presence. We simply select random 500 positively labeled samples for each of the 20 classes and learn 15 components. All of them are stacked together to create $\Va_{\text{train}}$.

\subsubsection{Hyperparameters} The hidden layers input to the interpreter module are selected from the convolutional block outputs. As is often the case with CNNs, the latter layers are expected to capture higher-order features. We thus select the last three convolutional block outputs as input to the network $\Psi$. The loss weights and number of components used for post-hoc interpretation are summarized in table \ref{hyperparams:ph}.

\begin{table}
    \setlength{\tabcolsep}{6pt}
	\centering
	%\small
    \resizebox{0.35\textwidth}{!}{%	
	\begin{tabular}{l c c c c} 
		\toprule
		  Dataset & $\alpha$ & $\beta$ & $K$ & \# of epochs \\ [0.5ex] 
		\midrule 
            ESC-50 & 10.0 & 0.8 & 100 & 35 \\
            %L3 \cite{lll} & 79.8 & $\times$ & $\times$ \\
            SONYC-UST & 10.0 & 0.8 & 80 & 21 \\
            OpenMIC-2018 & 5.0 & 0.2 & 300 & 21 \\
            \bottomrule
	\end{tabular}
     }
	\caption{Hyperparameters for all datasets for post-hoc interpretation}
    \label{hyperparams:ph}
\end{table}

\subsubsection{Optimization}

All the networks are optimized using Adam \cite{adam} with learning rate $2 \times 10^{-4}$. 



\subsection{Evaluated Systems}

We denote our proposed Listen to Interpret (L2I) system, with attention based pooling in $\Theta$ by L2I w/ $\Theta_{\textsc{att}}$. The most suitable baselines to benchmark its fidelity are \textit{post-hoc} methods that approximate the classifier over input space with a single surrogate model. We select two state-of-the-art systems, FLINT \cite{flint} and VIBI \cite{vibi}. A variant of our own proposed method, L2I w/ $\Theta_{\textsc{max}}$, is also evaluated. Herein, attention is replaced with 1D max-pooling operation.
% \ref{baseline_impl}

\textit{Faithfulness benchmarking}: As already discussed, it is not possible to measure faithfulness for concept-based \textit{post-hoc} interpretability approaches. While measurement for input attribution based approaches is possible, the interpretations themselves and the feature removal strategies are different, making comparisons with our system significantly less meaningful. We thus compare our faithfulness against a \textit{Random Baseline}, wherein the less-important components, those not present in $L_{c,x}$, are randomly removed. To compare fairly, we remove the same number of components that are present in $L_{c, x}$ on average. This would validate that, if the interpreter selects \textit{truly} important components for the classifier's decision, then randomly removing the less important ones should not cause a drop in the predicted class probability.

We also emphasize at this point that works related to audio interpretability (see Sec. \ref{related:audio_intp}), are not suitable for comparison on these metrics. Particularly, APNet \cite{apnet} is not designed for \textit{post-hoc} interpretations. AudioLIME \cite{aud-lime-1} is not applicable on our tasks as it requires known predefined audio sources. Moreover, SLIME \cite{slime-2} and AudioLIME still rely on LIME \cite{lime} for interpretations. It is a feature-attribution method that approximates a classifier for \textit{each} sample separately. As discussed before, these characteristics are not suitable for comparison on our metrics.



\subsection{Results}
\subsubsection{Fidelity}
As discussed previously, to quantify fidelity, we use the same respective metrics as done to benchmark classifier performance but evaluate them for interpreter output w.r.t classifier output. For ESC-50, mean and standard deviation of top-$k$ fidelity is calculated over the 5 folds. We show these results for $k=1, 5$.  %For fidelity, performance of our proposed system and its variants is comparable to that of FLINT. 
%This experiment serves as a sanity check for our system, that while achieving fidelity performance comparable to state-of-the-art, we hold the advantage of providing listenable interpretations in terms of pre--learnt spectral patterns.
For SONYC-UST, we report the macro-AUPRC, micro-AUPRC and max-F1 for the interpreter output w.r.t classifier. For fairness, we ignore the class `non-machinery impact' from all class-wise evaluations involved in fidelity (\textit{i.e.} macro-AUPRC) or faithfulness. This is because the classifier predicts only one sample in test set with positive label for this class, causing AUPRC scores to vary widely for different interpreters. %We suspect that our proposed L2I systems are better at handling noisy audio. In that, our NMF-styled decoder contains certain components that model noise and do not affect interpretations. In contrast, the attributes in FLINT are completely learnt and lack such well-defined structure. 
For OpenMIC-2018, we report the Fidelity weighted F1-score for each system. All the above results are available in Tab. \ref{fidelity_all}. 

Among the four systems, VIBI performs the worst in terms of fidelity. This is very likely because it treats the classifier as a black-box, while the other three systems access its hidden representations. This strongly indicates that accessing hidden layers can be beneficial for fidelity of interpreters. While on ESC50, FLINT achieves the best fidelity, L2I w/ $\Theta_{\text{ATT}}$ outperforms all systems on the other datasets. It should be noted that our system variants distinctly hold the advantage of generating listenable interpretations over FLINT and VIBI. Nevertheless, these systems form strong baselines for fidelity and the results demonstrate that our interpreter can generate high-fidelity \textit{post-hoc} interpretations. Moreover, its design is flexible w.r.t different pooling functions.


\begin{table*}
    \setlength{\tabcolsep}{7pt}
	\centering
	%\small
    \resizebox{0.87\textwidth}{!}{%	
	\begin{tabular}{l c c c c c} 
		\toprule
		& \multicolumn{2}{c}{ESC-50 (in \%)} & \multicolumn{2}{c}{SONYC-UST} & \multicolumn{1}{c}{OpenMIC-2018}\\
		\cmidrule[1pt](lr){2-3}
            \cmidrule[1pt](lr){4-5}
            \cmidrule[1pt](lr){6-6}
		System & top-1 & top-5 & macro-AUPRC & micro-AUPRC & avg-weighted-F1 \\ [0.5ex] 
		\midrule
		L2I w/ $\Theta_{\textsc{att}}$ & 65.7 $\pm$ 2.8 & 88.2 $\pm$ 1.7 & \bf{0.909 $\pm$ 0.011} & \bf{0.917 $\pm$ 0.008} & \bf{0.920 $\pm$ 0.004} \\ 
            L2I w/ $\Theta_{\textsc{max}}$ & 73.3 $\pm$ 2.3 & 92.7 $\pm$ 1.2 & 0.866 $\pm$ 0.014  & 0.913 $\pm$ 0.012 & 0.906 $\pm$ 0.004 \\
            \midrule
            FLINT \cite{flint} & \bf{73.5 $\pm$ 2.3} & \bf{93.4 $\pm$ 0.9} & 0.816 $\pm$ 0.013 & 0.907 $\pm$ 0.011 & 0.907 $\pm$ 0.004 \\
            VIBI \cite{vibi} & 27.7 $\pm$ 2.3 & 53.0 $\pm$ 1.8 & 0.608 $\pm$ 0.027  & 0.575 $\pm$ 0.019 & 0.581 $\pm$ 0.037 \\
 		\bottomrule
	\end{tabular}
     }
	%\vspace{-3pt}
	\caption{Fidelity results for the interpreter w.r.t classifier's output on all datasets. We report top-1 and top-5 fidelity (in \%) for ESC-50 (all five folds), AUPRC-based metrics for SONYC-UST and weighted F1-score averaged over all classes for OpenMIC-2018. All results contain mean and variance over three runs. Values in bold indicate maximum of the metric among all the evaluated systems (incl. baselines).}
	%\vspace{-14pt}
    \label{fidelity_all}
\end{table*}



\subsubsection{Faithfulness}
In Table \ref{faithfulness_esc50}, we report median faithfulness $\textrm{FF}_{\textrm{median}}$ on ESC-50 for our primary system L2I w/ $\Theta_{\textsc{ATT}}$ at different thresholds $\tau$ averaged over the five folds. Smaller $\tau$ corresponds to higher $|L_{c, x}|$, which denotes the number of components being used for generating interpretations. Thus, for Random Baseline, we report $\textrm{FF}_{\textrm{median}}$ at the lowest threshold $\tau=0.1$, to ensure removal of maximal number of components. To recall the definition of Random Baseline, please refer to Sec. \ref{metrics}. $\textrm{FF}_{\textrm{median}}$ for L2I w/ $\Theta_{\textsc{ATT}}$ is positive for all thresholds. It is also significantly higher than the Random Baseline, indicating faithfulness of interpretations.

The results for class-wise faithfulness on SONYC-UST and OpenMIC are illustrated in Fig. \ref{fig_faithfulness_sony} and \ref{fig_faithfulness_omic} respectively. We show $\textrm{FF}_{\text{median}}$ (absolute drop in probability) for our system and the Random Baseline. For most classes, interpretations can be considered faithful, with a significantly positive median compared to random baseline results, which are very close to 0.

\begin{table}[!t]
\setlength{\tabcolsep}{7pt}
	\centering
	\resizebox{0.41\textwidth}{!}{%
	\begin{tabular}[t]{l c c} 
		\toprule
		System & Threshold $\tau$ & $\text{FF}_\text{median}$ \\ [0.5ex] 
		\midrule
		\multirow{ 5}{*}{L2I w/ $\Theta_{\textsc{att}}$} & $\tau=0.9$ &  0.002 \\
		 & $\tau=0.7$ &  0.004 \\
		 & $\tau=0.5$ & 0.012\\
		 & $\tau=0.3$ &  0.040\\
		 & $\tau=0.1$ &  0.113\\
		\midrule
		Random Baseline & $\tau=0.1$ & $<10^{-4}$ \\
		\bottomrule\\
	\end{tabular}}
	%\vspace{-1pt}
	\caption{Faithfulness results on ESC-50 for different thresholds, $\tau$. We report $\text{FF}_\text{median}$ for proposed L2I w/ $\Theta_{\textsc{att}}$ and the Random Baseline.}
	%\vspace{-10pt}
    \label{faithfulness_esc50}
\end{table}

\begin{figure}[!t]
\centering
\includegraphics[width=0.44\textwidth]{figures/FFplot_SONYC_UST_v3.png}
\caption{Faithfulness (absolute drop in probability value) results for SONYC-UST arranged class-wise for threshold, $\tau=0.1$}
\label{fig_faithfulness_sony}
\end{figure}

\begin{figure}[!t]
\centering
\includegraphics[width=0.50\textwidth]{figures/FFplot_OpenMIC.png}
\caption{Faithfulness (absolute drop in probability value) results for OpenMIC-2018 arranged class-wise for threshold, $\tau=0.1$}
\label{fig_faithfulness_omic}
\end{figure}

\subsubsection{Subjective evaluation} We perform a user study (15 participants) to evaluate quality and understandability of interpretations for L2I against SLIME on SONYC-UST test data. As discussed previously, SLIME is not suitable for comparison on our quantitative metrics. Nevertheless, it is the only relevant baseline for qualitative study of listenable interpretations. Details about SLIME implementation are in supplement Sec. A.1.6. A participant was provided with 10 input samples, a predicted class by the classifier for each sample and the corresponding interpretation audios from SLIME and L2I. They were asked to rate the interpretations on a scale of 0-100 for the following question: ``\textit{How well does the interpretation correspond to the part of input audio associated with the given class?}". The 10 samples were randomly selected from a set of 36 (5-6 random test examples per class). For each sample, we ensured that the predicted class was both, present in the ground-truth and audible in input. 
Class-wise preference results and average ratings are shown in Fig. \ref{fig_sub_eval}. L2I is preferred for 'music', 'dog' \& 'alert-signal', SLIME is preferred for 'machinery-impact', no clear preference for others.

\begin{figure}[!t]
\centering
\includegraphics[width=0.48\textwidth]{figures/sub_eval_results_v2.png}
\caption{Subjective evaluation results. Average scores for L2I and SLIME and fraction of votes in favour of each system}
\label{fig_sub_eval}
\end{figure}



\subsection{Qualitative observations}
Qualitatively we observe that our interpretations are capable of emphasizing the object of interest and are insightful for an end-user to understand the classifier's prediction. We share multiple examples on our companion website.\footnote{\url{https://listen2interpret.000webhostapp.com/} \label{footnote 1}} Samples in case of SONYC-UST and OpenMIC are often already challenging with the presence of noise, or audio from other instruments respectively. In case of ESC50, to create more interesting and challenging scenarios we devise an experiment described below

\noindent \textbf{Audio corruption experiment: interpretability illustration}.~  For ESC50, we generate interpretations after corrupting the testing data for fold--1 in two different ways (i) either with white noise at 0dB SNR (signal-to-noise ratio), (ii) or mixing it with a sample of a different class. It should be noted that in both these cases the system is exactly the same as before and \textbf{not} trained with corrupted samples. Some examples, covering both types of corruptions are shared on our companion website.\textsuperscript{\ref{footnote 1}}. %A detailed qualitative analysis of this experiment can be found in supplement Sec. A.1.5.

For SONYC-UST, we observe good interpretations for classes `alert-signal', `dog' and `music'. For them, the background noise is significantly suppressed and the interpretations mainly focus on the object of interest. Interpretations for class `human' are also able to suppress noise to a certain extent and focus on parts of human voices. However, for this class, we found presence of some signal from other audio sources too. %However, some signal from other audio sources might also be present in the interpretations. 
For the remaining classes, namely `Engine', `Powered-saw' and 'Machinery-impact' the quality of the interpretation is more sample dependent. This is due to their acoustic similarity with the background noise. We provide example interpretations for SONYC-UST on our companion website.\textsuperscript{\ref{footnote 1}} 

The third dataset OpenMIC-2018, offers challenges under unique scenarios. Unlike SONYC-UST while it does not face issue of noise in data, it faces the hurdle of a strong overlap between instruments. This is because their onsets are often aligned by beats of the musical piece. This increases difficulty of filtering the signal of interest. Even with the greater complexity, the interpretations in many cases are able to emphasize the class of interest. Classes with relatively unique sounds such as `Bass' or `Mallet-percussion' are very well extracted. String like instruments including Violin and Guitar are also generally emphasized well.    

\noindent \textbf{Coherence of interpretations}.~ We visualize interpretations generated on the test set for SONYC-UST and OpenMIC-2018 by clustering relevance vectors. Specifically, we compute the vector $r_{c, x} \in \mathbb{R}^K$ which contains relevances of all components in prediction for class $c$ for sample $x$. The relevance vectors are collected for each test sample $x$ and its predicted class $c$. We then apply a t-SNE \cite{tsne} transformation to 2D for visualization. This is shown in Fig. \ref{tsne_rel}. Each point is labeled/colored according to the class for which we generate the interpretation. Interpretations for any single class are coherent and similar to each other. This is to some extent a positive consequence of global weight matrix in $\Theta$. Moreover, globally it can be observed that classes like 'Machinery-impact' and 'Powered-Saw' have similar relevances which are to some extent close to 'Engine'. This is to be expected as these classes are acoustically similar. 'Dog' and 'Music' are also close in this space, likely due to the often periodic nature of barks or beats. The visualization for OpenMIC is arguably even more interesting because of larger number of classes and several inter-class relationships. Various sets of similar instruments end-up as clusters in proximity of each other. The examples include `Cello-Violin', `Drums-Cymbals', `Clarinet-Flute', `Ukulele-Mandolin-Banjo', `Trombone-Trumpet-Saxophone'. Moreover, the meaningfulness of clustering also extends to higher-level of grouping. For example, the data is partitioned so as the string-based, wind-based, or percussion instruments are close to each other within their respective groups. This indicates that the interpreter's representations of what constitutes sound of an instrument aligns to some extent to human understanding. 

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.94\columnwidth]{figures_supplementary/clustering_intp.png}
    \includegraphics[width=0.96\columnwidth]{figures/omic_clustering_exp_v4.png}
    \caption{Visualized relevances (following a t-SNE transformation) of generated interpretations on test sets of SONYC-UST (top) and OpenMIC-2018 (bottom), colour-coded according to interpreted class. For clarity in case of OpenMIC, we show up to random 25 interpretations of a class.}
    \label{tsne_rel}
\end{figure}

\subsection{Ablation studies} 

Tab. \ref{ablation_hidden_layer} and Tab. \ref{ablation_loss} present ablation studies for loss hyperparameters and choice of hidden layers. The choices in bold indicate our current choices. The metrics and loss values given here are for a single run.

\begin{table}[!t]
\setlength{\tabcolsep}{8pt}
	\centering
	\resizebox{0.38\textwidth}{!}{%
	\begin{tabular}{l c c c} 
		\toprule
		ConvBlocks & $\bmL_{\textrm{NMF}}$ & $\bmL_{\textrm{FID}}$ & top-1 \\ [0.5ex] 
		\midrule
          %B2 & 0.091 & 2.065 & 49.0 \\
          B3 & 0.104 & 1.788 & 53.0 \\
          B6 & 0.118 & 1.698 & 57.8\\
          B2+B3 & 0.093 & 1.966 & 51.8 \\
		 B5+B6 & 0.103 & 1.572 & 61.5 \\
          \textbf{B4+B5+B6} & \textbf{0.079} & \textbf{1.546} & \textbf{65.5} \\
          \midrule
		 Input & 0.102 & 2.384 & 34.5\\
		\bottomrule\\
	\end{tabular}}
	%\vspace{-1pt}
	\caption{Ablation study for hidden layers: loss values on ESC50 (fold 1) test set for different subsets of hidden layers. Current choice indicated in bold.}
    \label{ablation_hidden_layer}
\end{table}


\begin{table}[!t]
\setlength{\tabcolsep}{7pt}
	\centering
	\resizebox{0.44\textwidth}{!}{%
	\begin{tabular}{c c c c c} 
		\toprule
		$\alpha$ & $\beta$ & $\bmL_{\textrm{NMF}}$ & $\bmL_{\textrm{FID}}$ & macro-AUPRC \\ [0.5ex] 
		\midrule
		 \textbf{10.0} & \textbf{0.8} & \textbf{0.028} & \textbf{0.386} & \textbf{0.900}\\
		 10.0 & 8.0 & 0.048 & 0.386 & 0.879\\
         10.0 & 0.08 & 0.028 & 0.388 & 0.876\\
         1.0 & 0.8 & 0.045 & 0.375 & 0.921\\
         100.0 & 0.8 & 0.027 & 0.445 & 0.612\\
		\bottomrule\\
	\end{tabular}}
	%\vspace{-1pt}
	\caption{Ablation study for loss hyperparameters: loss values on SONCY-UST test set for different weights of loss functions. Current choice indicated in bold.}
    \label{ablation_loss}
\end{table}

\noindent \textbf{Hidden layer selection} Deciding the hidden layers of the classifier that should be accessed by the interpreter is an important choice. At first glance, this might appear to be computationally too expensive as total possible choices is exponential in number of hidden layers. However, practical considerations can heavily reduce the search space. An upper bound to the number of layers could be set depending upon the desired size of interpreter. In our experiments throughout the paper, we limited ourselves to at most 3 layers. Crucially, layers close to the output are more favourable, for multiple reasons. They generally result in better fidelity and inherently tie the interpreter much closer to the output of classifier. Moreover, the latter layers are also expected to capture higher level features. We illustrate how selecting different subsets of hidden layers affects optimization of our fidelity and reconstruction loss by doing an ablation study. It's results are reported in table \ref{ablation_hidden_layer}. The classifier consists of 6 major convolutional blocks (B1--B6).

\noindent \textbf{Loss weights} We illustrate the effect of varying loss weights on optimization in table \ref{ablation_loss}. Too high emphasis on $\bmL_{\textrm{NMF}}$, that is, high $\alpha$ can hurt the fidelity of interpreter while a high $\beta$ (sparsity loss) can result in poorer reconstruction. Importantly, there is a good range of values wherein the system can be regarded as operating reasonably. 

\noindent \textbf{Number of components} Choice of number of components, $K$, also known as order estimation, is typically data and application dependent. It controls the granularity of the discovered audio spectral patterns. 
Choosing $K$ has also been a long standing problem within the NMF community \cite{tan2012automatic}. Our choice for this parameter was guided by three main factors: 
\begin{itemize}
    \item Choices made previously in literature for similar pre-learning of $\mathbf{W}$ \cite{bisot2017feature}, who demonstrated reasonable acoustic scene classification results with a dictionary size of $K=128$. We used this as a reference to guide our choice for number of components.
    \item Dataset specific details which include number of classes, samples for each class, variability of recordings etc. For eg. acoustic variability of ESC-50 (larger number of classes), prompted us to use a dictionary of larger size compared to SONYC-UST. We use highest number of components for OpenMIC, which has largest dataset size among the three and reasonably high acoustic variability.  
    \item When tracking loss values for different $K$, we observed a plateauing effect for larger dictionary sizes as illustrated in Fig. \ref{fig_loss_vs_K} for ESC-50 and OpenMIC-2018. In case of OpenMIC, this effect is prominent for reconstruction loss $\bmL_{\text{NMF}}$. The fidelity remains high even for small $K$ . 
\end{itemize}

\begin{figure}
    \centering
    \includegraphics[width=0.361\columnwidth]{figures/loss_vs_K_updated.png}
    ~
    \includegraphics[width=0.602\columnwidth]{figures/loss_vs_K_OpenMIC.png}
    \caption{Ablation study for number of components. Loss values on test data for ESC-50 and OpenMIC-2018.}
    \label{fig_loss_vs_K}
\end{figure}

%\subsection{Additional Exp 2}





% \begin{table*}[!t]
% \setlength{\tabcolsep}{3pt}
% 	\centering
% 	%\small
% \resizebox{0.5\textwidth}{!}{%	
% 	\begin{tabular}{l c c c} 
% 		\toprule
% 		& \multicolumn{3}{c}{Fidelity}\\
% 		\cmidrule[1pt](lr){2-4} 
% 		System & macro-AUPRC & micro-AUPRC & max-F1 \\ [0.5ex] 
% 		\midrule
% 		L2I + $\Theta_{\textsc{att}}$ & 0.909 $\pm$ 0.011  & 0.917 $\pm$ 0.008 & 0.847 $\pm$ 0.010 \\ 
% 		L2I + $\Theta_{\textsc{max}}$ & 0.866 $\pm$ 0.014  & 0.913 $\pm$ 0.012 & 0.840 $\pm$ 0.012  \\
% 		\midrule
% 	    FLINT & 0.816 $\pm$ 0.013 & 0.907 $\pm$ 0.011  & 0.825 $\pm$ 0.012 \\
%         VIBI  & 0.608 $\pm$ 0.027  & 0.575 $\pm$ 0.019 & 0.549 $\pm$ 0.020 \\
%  		\bottomrule\\
% 	\end{tabular}
% 	}
% 	%\vspace{-3pt}
% 	\caption{Fidelity results on SONYC-UST multi-label urban sound tagging task. We report AUPRC-based metrics and max F1 score for the interpreter w.r.t classifier's output (over three runs).}
% 	%\vspace{-14pt}
%     \label{fidelity_sonycust}
% \end{table*}

% \begin{table}[!t]
% \setlength{\tabcolsep}{3pt}
% 	\centering
% 	%\small
% \resizebox{0.24\textwidth}{!}{%	
% 	\begin{tabular}{l c} 
% 		\toprule
% 		& \multicolumn{1}{c}{Fidelity}\\
% 		\cmidrule[1pt](lr){2-2} 
% 		System & avg-weighted-F1 \\ [0.5ex] 
% 		\midrule
% 		L2I + $\Theta_{\textsc{att}}$ & 0.920 $\pm$ 0.004 \\ 
% 		L2I + $\Theta_{\textsc{max}}$ & 0.906 $\pm$ 0.004 \\
% 		\midrule
% 	    FLINT & 0.907 $\pm$ 0.004 \\
%         VIBI  & 0.581 $\pm$ 0.037  \\
%  		\bottomrule\\
% 	\end{tabular}
% 	}
% 	%\vspace{-3pt}
% 	\caption{Fidelity results on OpenMIC-2018 multi-label music instrument tagging task. We report weighted F1 score averaged over all classes for the interpreter w.r.t classifier's output (over three runs).}
%     \label{fidelity_openmic}
% \end{table}

